Simulations agree: the Milky Way's satellites are disrupting

Recent analyses of simulated Milky Way-mass galaxies have highlighted the prevalence of satellites undergoing tidal disruption. However, these have focused on single hydrodynamical codes with a number of limitations, making it unclear how generic this result is. We compare satellite disruption in four models: two cosmological hydrodynamical simulations (Auriga and FIRE), cosmological $N$-body simulations with stellar particle tagging (Aquarius), and a semi-analytic model with varying host disk properties (SatGen). For all systems, we compute the fraction of stellar mass retained by the progenitor ($f_\text{bound}$) at the present day. We find a remarkable agreement between FIRE, Aquarius, and SatGen; all predict that $\sim$20 to 30 per cent of classical-mass satellites have $f_\text{bound} < 0.9$ ($\sim$5 to 10 per cent have $f_\text{bound} < 0.5$). Satellites in Auriga experience substantially more mass loss than other simulations, which we attribute to their massive central galaxies and large satellite sizes prior to infall. In the ultra-faint regime captured by Aquarius and SatGen, disruption rates are comparable to or exceeding those for classical satellites. The ubiquity of mass loss across models presents both an exciting opportunity (a plethora of stellar streams awaiting discovery) and a nuisance (for theorists using satellite counts to constrain dark matter).

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

